From Templates to Natural Language: Generalization Challenges in Instruction-Tuned LLMs for Spatial Reasoning

Instruction-tuned large language models (LLMs) have shown strong performance on a variety of tasks; however, generalizing from synthetic to human-authored instructions in grounded environments remains a challenge for them. In this work, we study generalization challenges in spatial grounding tasks where models interpret and translate instructions for building object arrangements on a $2.5$D grid. We fine-tune LLMs using only synthetic instructions and evaluate their performance on a benchmark dataset containing both synthetic and human-written instructions. Our results reveal that while models generalize well on simple tasks, their performance degrades significantly on more complex tasks. We present a detailed error analysis of the gaps in instruction generalization.

==> latex/templates/instruction_similarity_shapewise.tex <==
\begin{table}
  \centering
  \small
  \begin{tabular}{ccccc}
    \hline
    \textbf{Score Ranges} & \multicolumn{2}{c}{\textbf{BLEU}} & \multicolumn{2}{c}{\textbf{ES}} \\
    & SB & RB & SB & RB \\
    \hline
    Median Values     & {0.356} & {0.024} & {0.979} & {0.623}           \\
    Min-Max Range     & {0.356} & {0.024} & {0.979} & {0.623}           \\
    \hline
  \end{tabular}
  \caption{\todo{placeholder table}}
  \label{tab:instruction_similarity_shapewise}
\end{table}
